Intelligent Communication Planning for Constrained Environmental IoT Sensing with Reinforcement Learning

Internet of Things (IoT) technologies have enabled numerous data-driven mobile applications and have the potential to significantly improve environmental monitoring and hazard warnings through the deployment of a network of IoT sensors. However, these IoT devices are often power-constrained and utilize wireless communication schemes with limited bandwidth. Such power constraints limit the amount of information each device can share across the network, while bandwidth limitations hinder sensors' coordination of their transmissions. In this work, we formulate the communication planning problem of IoT sensors that track the state of the environment. We seek to optimize sensors' decisions in collecting environmental data under stringent resource constraints. We propose a multi-agent reinforcement learning (MARL) method to find the optimal communication policies for each sensor that maximize the tracking accuracy subject to the power and bandwidth limitations. MARL learns and exploits the spatial-temporal correlation of the environmental data at each sensor's location to reduce the redundant reports from the sensors. Experiments on wildfire spread with LoRA wireless network simulators show that our MARL method can learn to balance the need to collect enough data to predict wildfire spread with unknown bandwidth limitations.

==> old_03_system.tex <==
\section{\sname{} System Design}\label{sec:system}
%\carlee{It's not that clear why this is separate from Section III on wildfire tracking. I would make the current Section III a subsection here (maybe replacing the current III-A on LoRA). We can also call the section ``System Design'' instead of Model.}
The objective of \sname{} is to develop efficient communication policies for IoT sensing. For the wildfire tracking problem, the goal is to improve the accuracy of the wildfire spread prediction by optimizing the communication policies of sensors  subject to power and bandwidth constraints. We use MARL  to automatically  learn  better communication patterns customized to the wildfire tracking problem.  The design of \sname{} is based on the following principles:
\begin{itemize}
    \item Minimize sensor requirements and radio uptime, to conserve sensor battery usage.
    \item Exploit opportunities to send feedback to sensors so they decide when to transmit later.
    \item Incorporate spatio-temporal correlations in finding the most useful data at sensors and using it to predict wildfire spread.
\end{itemize}

\subsection{Background: Wildfire Tracking}
We consider an IoT sensing system  for  wildfire tracking, as illustrated in Fig. \ref{fig:system}, composed of a set of IoT sensors,  a data fusion center and a  centralized communication layer. The sensors are spatially distributed across the area of fire potential and can sense the local fuel-weather-topography conditions in their immediate areas. For simplicity, we assume the sensor placement can cover the whole area of interest.  Each sensor has a local communication policy that determines when the sensor  communicates. The data fusion center, potentially cloud-based, collects local observation data from sensors and  predicts future fire spread. IoT sensors are connected to the fusion center through one or more gateways. 

\textbf{Sensor data collection:} Sensors are assumed to record the wind speed and direction of their local area at each time. \carlee{maybe put citations here?} They can also monitor a binary indicator of whether their current area is on fire or not (e.g., through temperature sensors). We assume that sensors do not store this data and only transmit the current sensed information to the fusion center, thus eliminating the need for a data queue at the sensors.

\textbf{Sensor communication:} We consider sensors that communicate with LoRa, which is one of the most prominent and revolutionary energy-efficient communication technologies for the IoT~\cite{lora-popularity}. LoRa enables extremely long-range and bidirectional communication between thousands of low-power  devices and always-on gateways, reducing the limitations from other wireless technologies (e.g., WiFi, Bluetooth) such as power and other overheads~\cite{iot_lora}. The MAC protocol stack, LoRaWAN, presents a  star-of-stars topology, where LoRa devices emit data packets and gateways receive those packets within their reception range. Packets may collide  with each other if they use the same carrier frequency and spreading factor with overlapping reception time. 
The gateway is registered to an application-server (data fusion center) to which it
transparently forwards all the received data. 
For downlink communication from the server, LoRa devices can open a reception window to receive downlink messages from the gateway in three different ways: (Type-A) after each transmission,  (Type-B)  at pre-scheduled times, and (Type-C) continously listening~\cite{lorawan}. Since we consider power-constrained devices, we assume Type A LoRa devices, which only receive a downlink message from the server after a successful transmission. Such bidirectional communication allows the data fusion center to  send  feedback to a subset of sensors to facilitate decision making of \sname{}'s learned MARL communication policies. 

% We assume the system operates in rounds. \carlee{If there is space, make this a list.} Within each round,  sensors first sense (observe) the surrounding local environment and decide whether or not to report the observations to the fusion center following the local MARL-trained communication policy. Then, the fusion center uses a wildfire predictor to incorporate newly reported data with historical observations to predict future wildfire growth, and send feedback to sensors that have just successfully reported. 

We assume the system operates in rounds.  Within each round, the following operations are performed in order:
\begin{itemize}
    \item Sensors observe the surrounding local environment.
    \item Following the local MARL-trained communication policy, each sensor decides whether or not to report the observations to the fusion center, and acts accordingly.
    \item The fusion center uses a wildfire predictor to incorporate newly reported data with historical observations to predict future wildfire growth.
    \item  The fusion center sends feedback to sensors that have just successfully reported. 
\end{itemize}


% \subsection{Communication layer: LoRa}\label{sec:lora}
% \carlee{I think this subsection can go in the evaluation, as it's not specific to the system design and we don't use these details in the MARL.}
%     Our  LoRa simulation  is based on LoRaSim,  one of the most popular simulators for LoRa/LoRaWAN ~\cite{lorasim}.  Key aspects of the physical layer (PHY) and the medium-access-control (MAC) layer of the LoRaWAN protocol are considered.  At the PHY layer,  the signal propagation follows the log-distance path loss model. At the MAC layer, the simulator reproduces the ALOHA-based access protocol adopted by LoRaWAN and  implements the Adaptive Data Rate (ADR) scheme that aims to optimize the data rate of the end devices by monitoring the channel conditions. 

\subsection{Wildfire Spread Model}\label{sec:wildfire}
\sname{}'s fusion center runs a fire spread prediction model that takes as input sensor readings and outputs a forecast of future wildfire spread.
Methods for predicting the fire spread are largely based on Rothermel's work~\cite{rothermel72} and the resulting Rothermel Model~\cite{rothermel1983predict}, which predicts fire behaviors by estimating the rate of spread (ROS) given  fuel-weather-topography conditions. Xu \cite{Xu} summarizes earlier  work and proposes a modeling framework that integrates geographic information system (GIS) and remote sensing, which lays the basis for modern wildfire simulation tools like BehavePlus~\cite{Heinsch2010BehavePlusFM} and FARSITE~\cite{united2015farsite}.   


 The fire modeling consists of two parts: a fire media module and a fire motion module. The \textit{media module} takes as input the maps of the fire behavior fuel models (defined by USDA Forest Service~\cite{scott2005standard}), fuel moisture, wind speed and direction, and topographic elevation and slope, and produces ROS maps that determine in what direction and at what speed the fire propagates.   The \textit{motion model} takes the ROS maps from the media module as input and generates a map of the cumulative time of spread. Details on the fire spread models and fuel models can be found in the references.  
 
\sname{} uses the wildfire modeling tool provided in GRASS GIS~\cite{neteler2012grass} for wildfire spread prediction. We assume prior knowledge of the local fuel models, moisture distribution and terrain (i.e., elevation and slope). The predictor  incorporates reported observations of local wind data and the binary burning indicators from sensors, and predicts future fire spread. It outputs the time each location starts burning for a given time period. Fig. \ref{fig:wildfire} shows an example of wildfire spread modeling.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/marl.pdf}
    \caption{MARL framework}
    \label{fig:marl}
\end{figure}


\section{MARL Framework}\label{sec:marl}

global information embedding + local policy network

offline training + online deployment

refer to Section \ref{sec:marl}
Consider $n$ nodes in an IoT network. In the RL framework, we define $S=\{s_i\}_{i=1}^{n}$ and $A=\{a_i\}_{i=1}^{n}$ as the global state and action, where $s_i$ and $a_i$ are respectively the local state and action of node $i$. Our goal is to maximize the global reward $R(S,A)$, where $R$ is the reward function determined by the global objective of the system. Due to the huge number of nodes in the IoT network, the global state/action space could be exponentially large, which is intractable by any single-agent RL method using a single model (e.g., neural network) to make decisions for all nodes. Instead, we consider each node $i$ as an agent that runs its own policy $\pi_i$. As discussed before, collaboration between nearby nodes could help them optimize their policies more efficiently, thus the local policy $\pi_i$ may not only depend on $s_i$, but also $\{s_j\}_{j\in N_i}$, where $N_i$ is the neighborhood of node $i$. We define $r_i$ as the local reward of agent $i$. which is affected by the local objective and competition (different nodes can have different objectives and the actions of other nodes could hinder one from achieving its objective). Our distributed RL framework will let each agent $i$ optimize its policy $\pi_i: \{s_j\}_{j\in N_i} \to a_i$, based on its local reward signal $r_i$. With the optimal local policies of all agents, the global reward $R(S, A)$ should also be maximized.
\begin{itemize}
    \item GNN (encoder)
    \item Policy Network
    \begin{enumerate}
        \item state
        \item action
        \item reward
    \end{enumerate}
\end{itemize}

